Magnetic Topological Quantum Chemistry

For over 100 years, the group-theoretic characterization of crystalline solids has provided the foundational language for diverse problems in physics and chemistry. However, the group theory of crystals with commensurate magnetic order has remained incomplete for the past 70 years, due to the complicated symmetries of magnetic crystals. In this work, we complete the 100-year-old problem of crystalline group theory by deriving the small corepresentations, momentum stars, compatibility relations, and magnetic elementary band corepresentations of the 1,421 magnetic space groups (MSGs), which we have made freely accessible through tools on the Bilbao Crystallographic Server. We extend Topological Quantum Chemistry to the MSGs to form a complete, real-space theory of band topology in magnetic and nonmagnetic crystalline solids - Magnetic Topological Quantum Chemistry (MTQC). Using MTQC, we derive the complete set of symmetry-based indicators of electronic band topology, for which we identify symmetry-respecting bulk and anomalous surface and hinge states.

==> dependencies.tex <==
\textbf{2.4}&$\mathbf{P\bar{1}}$&\textbf{I}&\textbf{2.4}&$\mathbf{P\bar{1}}$&\textbf{I}&\textbf{2.5}&$\mathbf{P\bar{1}1'}$&\textbf{II}&\textbf{2.5}&$\mathbf{P\bar{1}1'}$&\textbf{II}\\
\hline
2.7&$P_S\bar{1}$&IV&2.4&$P\bar{1}$&I&\textbf{3.1}&$\mathbf{P2}$&\textbf{I}&\textbf{3.1}&$\mathbf{P2}$&\textbf{I}\\
\hline
3.4&$P_a2$&IV&3.1&$P2$&I&\textbf{10.42}&$\mathbf{P2/m}$&\textbf{I}&\textbf{10.42}&$\mathbf{P2/m}$&\textbf{I}\\
\hline
10.43&$P2/m1'$&II&2.5&$P\bar{1}1'$&II&10.46&$P2'/m'$&III&2.4&$P\bar{1}$&I\\
\hline
10.47&$P_a2/m$&IV&10.42&$P2/m$&I&10.48&$P_b2/m$&IV&2.4&$P\bar{1}$&I\\
\hline
10.49&$P_C2/m$&IV&2.4&$P\bar{1}$&I&11.50&$P2_1/m$&I&2.4&$P\bar{1}$&I\\
\hline
11.51&$P2_1/m1'$&II&2.5&$P\bar{1}1'$&II&11.54&$P2_1'/m'$&III&2.4&$P\bar{1}$&I\\
\hline
11.55&$P_a2_1/m$&IV&2.4&$P\bar{1}$&I&11.56&$P_b2_1/m$&IV&2.4&$P\bar{1}$&I\\
\hline
11.57&$P_C2_1/m$&IV&2.4&$P\bar{1}$&I&12.58&$C2/m$&I&2.4&$P\bar{1}$&I\\
\hline
12.59&$C2/m1'$&II&2.5&$P\bar{1}1'$&II&12.62&$C2'/m'$&III&2.4&$P\bar{1}$&I\\
\hline
12.63&$C_c2/m$&IV&2.4&$P\bar{1}$&I&12.64&$C_a2/m$&IV&2.4&$P\bar{1}$&I\\
\hline
13.65&$P2/c$&I&2.4&$P\bar{1}$&I&13.66&$P2/c1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
13.69&$P2'/c'$&III&2.4&$P\bar{1}$&I&13.70&$P_a2/c$&IV&2.4&$P\bar{1}$&I\\
\hline
13.71&$P_b2/c$&IV&2.4&$P\bar{1}$&I&13.72&$P_c2/c$&IV&2.4&$P\bar{1}$&I\\
\hline
13.73&$P_A2/c$&IV&2.4&$P\bar{1}$&I&13.74&$P_C2/c$&IV&2.4&$P\bar{1}$&I\\
\hline
14.75&$P2_1/c$&I&2.4&$P\bar{1}$&I&14.76&$P2_1/c1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
14.79&$P2_1'/c'$&III&2.4&$P\bar{1}$&I&14.80&$P_a2_1/c$&IV&2.4&$P\bar{1}$&I\\
\hline
14.81&$P_b2_1/c$&IV&2.4&$P\bar{1}$&I&14.82&$P_c2_1/c$&IV&2.4&$P\bar{1}$&I\\
\hline
14.83&$P_A2_1/c$&IV&2.4&$P\bar{1}$&I&14.84&$P_C2_1/c$&IV&2.4&$P\bar{1}$&I\\
\hline
15.85&$C2/c$&I&2.4&$P\bar{1}$&I&15.86&$C2/c1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
15.89&$C2'/c'$&III&2.4&$P\bar{1}$&I&15.90&$C_c2/c$&IV&2.4&$P\bar{1}$&I\\
\hline
15.91&$C_a2/c$&IV&2.4&$P\bar{1}$&I&16.3&$P2'2'2$&III&3.1&$P2$&I\\
\hline
17.10&$P22'2_1'$&III&3.1&$P2$&I&18.18&$P2_1'2_1'2$&III&3.1&$P2$&I\\
\hline
21.40&$C2'2'2$&III&3.1&$P2$&I&25.60&$Pm'm'2$&III&3.1&$P2$&I\\
\hline
\textbf{27.81}&$\mathbf{Pc'c'2}$&\textbf{III}&\textbf{27.81}&$\mathbf{Pc'c'2}$&\textbf{III}&28.91&$Pm'a'2$&III&3.1&$P2$&I\\
\hline
30.117&$P_bnc2$&IV&27.81&$Pc'c'2$&III&32.138&$Pb'a'2$&III&3.1&$P2$&I\\
\hline
34.163&$P_Cnn2$&IV&27.81&$Pc'c'2$&III&35.168&$Cm'm'2$&III&3.1&$P2$&I\\
\hline
37.183&$Cc'c'2$&III&27.81&$Pc'c'2$&III&37.185&$C_acc2$&IV&27.81&$Pc'c'2$&III\\
\hline
39.199&$Ab'm'2$&III&27.81&$Pc'c'2$&III&\textbf{41.215}&$\mathbf{Ab'a'2}$&\textbf{III}&\textbf{41.215}&$\mathbf{Ab'a'2}$&\textbf{III}\\
\hline
42.222&$Fm'm'2$&III&27.81&$Pc'c'2$&III&45.238&$Ib'a'2$&III&27.81&$Pc'c'2$&III\\
\hline
\textbf{47.249}&$\mathbf{Pmmm}$&\textbf{I}&\textbf{47.249}&$\mathbf{Pmmm}$&\textbf{I}&47.250&$Pmmm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
47.252&$Pm'm'm$&III&10.42&$P2/m$&I&47.254&$P_ammm$&IV&47.249&$Pmmm$&I\\
\hline
47.255&$P_Cmmm$&IV&47.249&$Pmmm$&I&47.256&$P_Immm$&IV&47.249&$Pmmm$&I\\
\hline
48.257&$Pnnn$&I&2.4&$P\bar{1}$&I&48.258&$Pnnn1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
48.260&$Pn'n'n$&III&2.4&$P\bar{1}$&I&48.262&$P_cnnn$&IV&2.4&$P\bar{1}$&I\\
\hline
48.263&$P_Cnnn$&IV&2.4&$P\bar{1}$&I&48.264&$P_Innn$&IV&2.4&$P\bar{1}$&I\\
\hline
49.265&$Pccm$&I&2.4&$P\bar{1}$&I&49.266&$Pccm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
49.269&$Pc'c'm$&III&10.42&$P2/m$&I&49.270&$Pc'cm'$&III&2.4&$P\bar{1}$&I\\
\hline
49.272&$P_accm$&IV&2.4&$P\bar{1}$&I&49.273&$P_cccm$&IV&2.4&$P\bar{1}$&I\\
\hline
49.274&$P_Bccm$&IV&2.4&$P\bar{1}$&I&49.275&$P_Cccm$&IV&2.4&$P\bar{1}$&I\\
\hline
49.276&$P_Iccm$&IV&2.4&$P\bar{1}$&I&50.277&$Pban$&I&2.4&$P\bar{1}$&I\\
\hline
50.278&$Pban1'$&II&2.5&$P\bar{1}1'$&II&50.281&$Pb'a'n$&III&2.4&$P\bar{1}$&I\\
\hline
50.282&$Pb'an'$&III&2.4&$P\bar{1}$&I&50.284&$P_aban$&IV&2.4&$P\bar{1}$&I\\
\hline
50.285&$P_cban$&IV&2.4&$P\bar{1}$&I&50.286&$P_Aban$&IV&2.4&$P\bar{1}$&I\\
\hline
50.287&$P_Cban$&IV&2.4&$P\bar{1}$&I&50.288&$P_Iban$&IV&2.4&$P\bar{1}$&I\\
\hline
51.289&$Pmma$&I&10.42&$P2/m$&I&51.290&$Pmma1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
51.294&$Pm'm'a$&III&2.4&$P\bar{1}$&I&51.295&$Pmm'a'$&III&2.4&$P\bar{1}$&I\\
\hline
51.296&$Pm'ma'$&III&10.42&$P2/m$&I&51.298&$P_amma$&IV&10.42&$P2/m$&I\\
\hline
51.299&$P_bmma$&IV&2.4&$P\bar{1}$&I&51.300&$P_cmma$&IV&10.42&$P2/m$&I\\
\hline
51.301&$P_Amma$&IV&2.4&$P\bar{1}$&I&51.302&$P_Bmma$&IV&10.42&$P2/m$&I\\
\hline
51.303&$P_Cmma$&IV&2.4&$P\bar{1}$&I&51.304&$P_Imma$&IV&2.4&$P\bar{1}$&I\\
\hline
52.305&$Pnna$&I&2.4&$P\bar{1}$&I&52.306&$Pnna1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
52.310&$Pn'n'a$&III&2.4&$P\bar{1}$&I&52.311&$Pnn'a'$&III&2.4&$P\bar{1}$&I\\
\hline
52.312&$Pn'na'$&III&2.4&$P\bar{1}$&I&52.314&$P_anna$&IV&2.4&$P\bar{1}$&I\\
\hline
52.315&$P_bnna$&IV&2.4&$P\bar{1}$&I&52.316&$P_cnna$&IV&2.4&$P\bar{1}$&I\\
\hline
52.317&$P_Anna$&IV&2.4&$P\bar{1}$&I&52.318&$P_Bnna$&IV&2.4&$P\bar{1}$&I\\
\hline
52.319&$P_Cnna$&IV&2.4&$P\bar{1}$&I&52.320&$P_Inna$&IV&2.4&$P\bar{1}$&I\\
\hline
53.321&$Pmna$&I&2.4&$P\bar{1}$&I&53.322&$Pmna1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
53.326&$Pm'n'a$&III&2.4&$P\bar{1}$&I&53.327&$Pmn'a'$&III&10.42&$P2/m$&I\\
\hline
53.328&$Pm'na'$&III&2.4&$P\bar{1}$&I&53.330&$P_amna$&IV&2.4&$P\bar{1}$&I\\
\hline
53.331&$P_bmna$&IV&2.4&$P\bar{1}$&I&53.332&$P_cmna$&IV&2.4&$P\bar{1}$&I\\
\hline
53.333&$P_Amna$&IV&2.4&$P\bar{1}$&I&53.334&$P_Bmna$&IV&2.4&$P\bar{1}$&I\\
\hline
53.335&$P_Cmna$&IV&2.4&$P\bar{1}$&I&53.336&$P_Imna$&IV&2.4&$P\bar{1}$&I\\
\hline
54.337&$Pcca$&I&2.4&$P\bar{1}$&I&54.338&$Pcca1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
\textbf{54.342}&$\mathbf{Pc'c'a}$&\textbf{III}&\textbf{54.342}&$\mathbf{Pc'c'a}$&\textbf{III}&54.343&$Pcc'a'$&III&2.4&$P\bar{1}$&I\\
\hline
54.344&$Pc'ca'$&III&2.4&$P\bar{1}$&I&54.346&$P_acca$&IV&2.4&$P\bar{1}$&I\\
\hline
54.347&$P_bcca$&IV&2.4&$P\bar{1}$&I&54.348&$P_ccca$&IV&2.4&$P\bar{1}$&I\\
\hline
54.349&$P_Acca$&IV&2.4&$P\bar{1}$&I&54.350&$P_Bcca$&IV&2.4&$P\bar{1}$&I\\
\hline
54.351&$P_Ccca$&IV&2.4&$P\bar{1}$&I&54.352&$P_Icca$&IV&2.4&$P\bar{1}$&I\\
\hline
55.353&$Pbam$&I&10.42&$P2/m$&I&55.354&$Pbam1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
55.357&$Pb'a'm$&III&10.42&$P2/m$&I&55.358&$Pb'am'$&III&2.4&$P\bar{1}$&I\\
\hline
55.360&$P_abam$&IV&10.42&$P2/m$&I&55.361&$P_cbam$&IV&2.4&$P\bar{1}$&I\\
\hline
55.362&$P_Abam$&IV&2.4&$P\bar{1}$&I&55.363&$P_Cbam$&IV&10.42&$P2/m$&I\\
\hline
55.364&$P_Ibam$&IV&2.4&$P\bar{1}$&I&56.365&$Pccn$&I&2.4&$P\bar{1}$&I\\
\hline
56.366&$Pccn1'$&II&2.5&$P\bar{1}1'$&II&\textbf{56.369}&$\mathbf{Pc'c'n}$&\textbf{III}&\textbf{56.369}&$\mathbf{Pc'c'n}$&\textbf{III}\\
\hline
56.370&$Pc'cn'$&III&2.4&$P\bar{1}$&I&56.372&$P_bccn$&IV&2.4&$P\bar{1}$&I\\
\hline
56.373&$P_cccn$&IV&2.4&$P\bar{1}$&I&56.374&$P_Accn$&IV&2.4&$P\bar{1}$&I\\
\hline
56.375&$P_Cccn$&IV&2.4&$P\bar{1}$&I&56.376&$P_Iccn$&IV&2.4&$P\bar{1}$&I\\
\hline
57.377&$Pbcm$&I&2.4&$P\bar{1}$&I&57.378&$Pbcm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
57.382&$Pb'c'm$&III&2.4&$P\bar{1}$&I&57.383&$Pbc'm'$&III&2.4&$P\bar{1}$&I\\
\hline
57.384&$Pb'cm'$&III&2.4&$P\bar{1}$&I&57.386&$P_abcm$&IV&2.4&$P\bar{1}$&I\\
\hline
57.387&$P_bbcm$&IV&2.4&$P\bar{1}$&I&57.388&$P_cbcm$&IV&2.4&$P\bar{1}$&I\\
\hline
57.389&$P_Abcm$&IV&2.4&$P\bar{1}$&I&57.390&$P_Bbcm$&IV&2.4&$P\bar{1}$&I\\
\hline
57.391&$P_Cbcm$&IV&2.4&$P\bar{1}$&I&57.392&$P_Ibcm$&IV&2.4&$P\bar{1}$&I\\
\hline
58.393&$Pnnm$&I&2.4&$P\bar{1}$&I&58.394&$Pnnm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
58.397&$Pn'n'm$&III&10.42&$P2/m$&I&58.398&$Pnn'm'$&III&2.4&$P\bar{1}$&I\\
\hline
58.400&$P_annm$&IV&2.4&$P\bar{1}$&I&58.401&$P_cnnm$&IV&2.4&$P\bar{1}$&I\\
\hline
58.402&$P_Bnnm$&IV&2.4&$P\bar{1}$&I&58.403&$P_Cnnm$&IV&2.4&$P\bar{1}$&I\\
\hline
58.404&$P_Innm$&IV&2.4&$P\bar{1}$&I&59.405&$Pmmn$&I&2.4&$P\bar{1}$&I\\
\hline
59.406&$Pmmn1'$&II&2.5&$P\bar{1}1'$&II&59.409&$Pm'm'n$&III&2.4&$P\bar{1}$&I\\
\hline
59.410&$Pmm'n'$&III&2.4&$P\bar{1}$&I&59.412&$P_bmmn$&IV&2.4&$P\bar{1}$&I\\
\hline
59.413&$P_cmmn$&IV&2.4&$P\bar{1}$&I&59.414&$P_Bmmn$&IV&2.4&$P\bar{1}$&I\\
\hline
59.415&$P_Cmmn$&IV&2.4&$P\bar{1}$&I&59.416&$P_Immn$&IV&2.4&$P\bar{1}$&I\\
\hline
60.417&$Pbcn$&I&2.4&$P\bar{1}$&I&60.418&$Pbcn1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
60.422&$Pb'c'n$&III&2.4&$P\bar{1}$&I&60.423&$Pbc'n'$&III&2.4&$P\bar{1}$&I\\
\hline
\textbf{60.424}&$\mathbf{Pb'cn'}$&\textbf{III}&\textbf{60.424}&$\mathbf{Pb'cn'}$&\textbf{III}&60.426&$P_abcn$&IV&2.4&$P\bar{1}$&I\\
\hline
60.427&$P_bbcn$&IV&2.4&$P\bar{1}$&I&60.428&$P_cbcn$&IV&2.4&$P\bar{1}$&I\\
\hline
60.429&$P_Abcn$&IV&2.4&$P\bar{1}$&I&60.430&$P_Bbcn$&IV&2.4&$P\bar{1}$&I\\
\hline
60.431&$P_Cbcn$&IV&2.4&$P\bar{1}$&I&60.432&$P_Ibcn$&IV&2.4&$P\bar{1}$&I\\
\hline
61.433&$Pbca$&I&2.4&$P\bar{1}$&I&61.434&$Pbca1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
61.436&$Pb'c'a$&III&2.4&$P\bar{1}$&I&61.438&$P_abca$&IV&2.4&$P\bar{1}$&I\\
\hline
61.439&$P_Cbca$&IV&2.4&$P\bar{1}$&I&61.440&$P_Ibca$&IV&2.4&$P\bar{1}$&I\\
\hline
62.441&$Pnma$&I&2.4&$P\bar{1}$&I&62.442&$Pnma1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
62.446&$Pn'm'a$&III&2.4&$P\bar{1}$&I&62.447&$Pnm'a'$&III&2.4&$P\bar{1}$&I\\
\hline
62.448&$Pn'ma'$&III&2.4&$P\bar{1}$&I&62.450&$P_anma$&IV&2.4&$P\bar{1}$&I\\
\hline
62.451&$P_bnma$&IV&2.4&$P\bar{1}$&I&62.452&$P_cnma$&IV&2.4&$P\bar{1}$&I\\
\hline
62.453&$P_Anma$&IV&2.4&$P\bar{1}$&I&62.454&$P_Bnma$&IV&2.4&$P\bar{1}$&I\\
\hline
62.455&$P_Cnma$&IV&2.4&$P\bar{1}$&I&62.456&$P_Inma$&IV&2.4&$P\bar{1}$&I\\
\hline
63.457&$Cmcm$&I&2.4&$P\bar{1}$&I&63.458&$Cmcm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
63.462&$Cm'c'm$&III&2.4&$P\bar{1}$&I&63.463&$Cmc'm'$&III&2.4&$P\bar{1}$&I\\
\hline
63.464&$Cm'cm'$&III&2.4&$P\bar{1}$&I&63.466&$C_cmcm$&IV&2.4&$P\bar{1}$&I\\
\hline
63.467&$C_amcm$&IV&2.4&$P\bar{1}$&I&63.468&$C_Amcm$&IV&2.4&$P\bar{1}$&I\\
\hline
64.469&$Cmca$&I&2.4&$P\bar{1}$&I&64.470&$Cmca1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
64.474&$Cm'c'a$&III&2.4&$P\bar{1}$&I&64.475&$Cmc'a'$&III&2.4&$P\bar{1}$&I\\
\hline
64.476&$Cm'ca'$&III&2.4&$P\bar{1}$&I&64.478&$C_cmca$&IV&2.4&$P\bar{1}$&I\\
\hline
64.479&$C_amca$&IV&2.4&$P\bar{1}$&I&64.480&$C_Amca$&IV&2.4&$P\bar{1}$&I\\
\hline
65.481&$Cmmm$&I&47.249&$Pmmm$&I&65.482&$Cmmm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
65.485&$Cm'm'm$&III&10.42&$P2/m$&I&65.486&$Cmm'm'$&III&2.4&$P\bar{1}$&I\\
\hline
65.488&$C_cmmm$&IV&47.249&$Pmmm$&I&65.489&$C_ammm$&IV&47.249&$Pmmm$&I\\
\hline
65.490&$C_Ammm$&IV&47.249&$Pmmm$&I&66.491&$Cccm$&I&2.4&$P\bar{1}$&I\\
\hline
66.492&$Cccm1'$&II&2.5&$P\bar{1}1'$&II&66.495&$Cc'c'm$&III&10.42&$P2/m$&I\\
\hline
66.496&$Ccc'm'$&III&2.4&$P\bar{1}$&I&66.498&$C_cccm$&IV&2.4&$P\bar{1}$&I\\
\hline
66.499&$C_accm$&IV&2.4&$P\bar{1}$&I&66.500&$C_Accm$&IV&2.4&$P\bar{1}$&I\\
\hline
67.501&$Cmma$&I&2.4&$P\bar{1}$&I&67.502&$Cmma1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
67.505&$Cm'm'a$&III&2.4&$P\bar{1}$&I&67.506&$Cmm'a'$&III&2.4&$P\bar{1}$&I\\
\hline
67.508&$C_cmma$&IV&2.4&$P\bar{1}$&I&67.509&$C_amma$&IV&2.4&$P\bar{1}$&I\\
\hline
67.510&$C_Amma$&IV&2.4&$P\bar{1}$&I&68.511&$Ccca$&I&2.4&$P\bar{1}$&I\\
\hline
68.512&$Ccca1'$&II&2.5&$P\bar{1}1'$&II&68.515&$Cc'c'a$&III&54.342&$Pc'c'a$&III\\
\hline
68.516&$Ccc'a'$&III&2.4&$P\bar{1}$&I&68.518&$C_ccca$&IV&2.4&$P\bar{1}$&I\\
\hline
68.519&$C_acca$&IV&2.4&$P\bar{1}$&I&68.520&$C_Acca$&IV&2.4&$P\bar{1}$&I\\
\hline
69.521&$Fmmm$&I&47.249&$Pmmm$&I&69.522&$Fmmm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
69.524&$Fm'm'm$&III&2.4&$P\bar{1}$&I&69.526&$F_Smmm$&IV&47.249&$Pmmm$&I\\
\hline
70.527&$Fddd$&I&2.4&$P\bar{1}$&I&70.528&$Fddd1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
70.530&$Fd'd'd$&III&2.4&$P\bar{1}$&I&70.532&$F_Sddd$&IV&2.4&$P\bar{1}$&I\\
\hline
71.533&$Immm$&I&47.249&$Pmmm$&I&71.534&$Immm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
71.536&$Im'm'm$&III&2.4&$P\bar{1}$&I&71.538&$I_cmmm$&IV&47.249&$Pmmm$&I\\
\hline
72.539&$Ibam$&I&2.4&$P\bar{1}$&I&72.540&$Ibam1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
72.543&$Ib'a'm$&III&2.4&$P\bar{1}$&I&72.544&$Iba'm'$&III&2.4&$P\bar{1}$&I\\
\hline
72.546&$I_cbam$&IV&2.4&$P\bar{1}$&I&72.547&$I_bbam$&IV&2.4&$P\bar{1}$&I\\
\hline
73.548&$Ibca$&I&2.4&$P\bar{1}$&I&73.549&$Ibca1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
73.551&$Ib'c'a$&III&2.4&$P\bar{1}$&I&73.553&$I_cbca$&IV&2.4&$P\bar{1}$&I\\
\hline
74.554&$Imma$&I&2.4&$P\bar{1}$&I&74.555&$Imma1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
74.558&$Im'm'a$&III&2.4&$P\bar{1}$&I&74.559&$Imm'a'$&III&2.4&$P\bar{1}$&I\\
\hline
74.561&$I_cmma$&IV&2.4&$P\bar{1}$&I&74.562&$I_bmma$&IV&2.4&$P\bar{1}$&I\\
\hline
\textbf{75.1}&$\mathbf{P4}$&\textbf{I}&\textbf{75.1}&$\mathbf{P4}$&\textbf{I}&75.5&$P_C4$&IV&75.1&$P4$&I\\
\hline
\textbf{77.13}&$\mathbf{P4_2}$&\textbf{I}&\textbf{77.13}&$\mathbf{P4_2}$&\textbf{I}&77.17&$P_C4_2$&IV&77.13&$P4_2$&I\\
\hline
79.25&$I4$&I&75.1&$P4$&I&\textbf{81.33}&$\mathbf{P\bar{4}}$&\textbf{I}&\textbf{81.33}&$\mathbf{P\bar{4}}$&\textbf{I}\\
\hline
81.34&$P\bar{4}1'$&II&81.33&$P\bar{4}$&I&81.36&$P_c\bar{4}$&IV&81.33&$P\bar{4}$&I\\
\hline
81.37&$P_C\bar{4}$&IV&81.33&$P\bar{4}$&I&81.38&$P_I\bar{4}$&IV&81.33&$P\bar{4}$&I\\
\hline
82.39&$I\bar{4}$&I&81.33&$P\bar{4}$&I&82.40&$I\bar{4}1'$&II&81.33&$P\bar{4}$&I\\
\hline
82.42&$I_c\bar{4}$&IV&81.33&$P\bar{4}$&I&\textbf{83.43}&$\mathbf{P4/m}$&\textbf{I}&\textbf{83.43}&$\mathbf{P4/m}$&\textbf{I}\\
\hline
\textbf{83.44}&$\mathbf{P4/m1'}$&\textbf{II}&\textbf{83.44}&$\mathbf{P4/m1'}$&\textbf{II}&\textbf{83.45}&$\mathbf{P4'/m}$&\textbf{III}&\textbf{83.45}&$\mathbf{P4'/m}$&\textbf{III}\\
\hline
83.47&$P4'/m'$&III&81.33&$P\bar{4}$&I&83.48&$P_c4/m$&IV&83.43&$P4/m$&I\\
\hline
83.49&$P_C4/m$&IV&83.43&$P4/m$&I&83.50&$P_I4/m$&IV&83.43&$P4/m$&I\\
\hline
\textbf{84.51}&$\mathbf{P4_2/m}$&\textbf{I}&\textbf{84.51}&$\mathbf{P4_2/m}$&\textbf{I}&84.52&$P4_2/m1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
84.53&$P4_2'/m$&III&10.42&$P2/m$&I&84.55&$P4_2'/m'$&III&81.33&$P\bar{4}$&I\\
\hline
84.56&$P_c4_2/m$&IV&83.45&$P4'/m$&III&84.57&$P_C4_2/m$&IV&84.51&$P4_2/m$&I\\
\hline
84.58&$P_I4_2/m$&IV&83.45&$P4'/m$&III&85.59&$P4/n$&I&81.33&$P\bar{4}$&I\\
\hline
85.60&$P4/n1'$&II&2.5&$P\bar{1}1'$&II&85.61&$P4'/n$&III&2.4&$P\bar{1}$&I\\
\hline
85.63&$P4'/n'$&III&81.33&$P\bar{4}$&I&85.64&$P_c4/n$&IV&2.4&$P\bar{1}$&I\\
\hline
85.65&$P_C4/n$&IV&2.4&$P\bar{1}$&I&85.66&$P_I4/n$&IV&2.4&$P\bar{1}$&I\\
\hline
86.67&$P4_2/n$&I&81.33&$P\bar{4}$&I&86.68&$P4_2/n1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
86.69&$P4_2'/n$&III&2.4&$P\bar{1}$&I&86.71&$P4_2'/n'$&III&81.33&$P\bar{4}$&I\\
\hline
86.72&$P_c4_2/n$&IV&2.4&$P\bar{1}$&I&86.73&$P_C4_2/n$&IV&2.4&$P\bar{1}$&I\\
\hline
86.74&$P_I4_2/n$&IV&2.4&$P\bar{1}$&I&87.75&$I4/m$&I&83.43&$P4/m$&I\\
\hline
\textbf{87.76}&$\mathbf{I4/m1'}$&\textbf{II}&\textbf{87.76}&$\mathbf{I4/m1'}$&\textbf{II}&87.77&$I4'/m$&III&83.45&$P4'/m$&III\\
\hline
87.79&$I4'/m'$&III&81.33&$P\bar{4}$&I&87.80&$I_c4/m$&IV&83.43&$P4/m$&I\\
\hline
\textbf{88.81}&$\mathbf{I4_1/a}$&\textbf{I}&\textbf{88.81}&$\mathbf{I4_1/a}$&\textbf{I}&88.82&$I4_1/a1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
88.83&$I4_1'/a$&III&2.4&$P\bar{1}$&I&88.85&$I4_1'/a'$&III&81.33&$P\bar{4}$&I\\
\hline
88.86&$I_c4_1/a$&IV&2.4&$P\bar{1}$&I&89.90&$P42'2'$&III&75.1&$P4$&I\\
\hline
90.98&$P42_1'2'$&III&75.1&$P4$&I&93.122&$P4_22'2'$&III&77.13&$P4_2$&I\\
\hline
94.130&$P4_22_1'2'$&III&77.13&$P4_2$&I&97.154&$I42'2'$&III&75.1&$P4$&I\\
\hline
99.167&$P4m'm'$&III&75.1&$P4$&I&100.175&$P4b'm'$&III&75.1&$P4$&I\\
\hline
101.183&$P4_2c'm'$&III&27.81&$Pc'c'2$&III&102.191&$P4_2n'm'$&III&77.13&$P4_2$&I\\
\hline
\textbf{103.199}&$\mathbf{P4c'c'}$&\textbf{III}&\textbf{103.199}&$\mathbf{P4c'c'}$&\textbf{III}&104.207&$P4n'c'$&III&27.81&$Pc'c'2$&III\\
\hline
104.209&$P_C4nc$&IV&103.199&$P4c'c'$&III&105.215&$P4_2m'c'$&III&27.81&$Pc'c'2$&III\\
\hline
106.223&$P4_2b'c'$&III&27.81&$Pc'c'2$&III&107.231&$I4m'm'$&III&27.81&$Pc'c'2$&III\\
\hline
108.237&$I4c'm'$&III&103.199&$P4c'c'$&III&\textbf{110.249}&$\mathbf{I4_1c'd'}$&\textbf{III}&\textbf{110.249}&$\mathbf{I4_1c'd'}$&\textbf{III}\\
\hline
111.251&$P\bar{4}2m$&I&81.33&$P\bar{4}$&I&111.252&$P\bar{4}2m1'$&II&81.33&$P\bar{4}$&I\\
\hline
111.255&$P\bar{4}2'm'$&III&81.33&$P\bar{4}$&I&111.256&$P_c\bar{4}2m$&IV&81.33&$P\bar{4}$&I\\
\hline
111.257&$P_C\bar{4}2m$&IV&81.33&$P\bar{4}$&I&111.258&$P_I\bar{4}2m$&IV&81.33&$P\bar{4}$&I\\
\hline
112.259&$P\bar{4}2c$&I&81.33&$P\bar{4}$&I&112.260&$P\bar{4}2c1'$&II&81.33&$P\bar{4}$&I\\
\hline
112.263&$P\bar{4}2'c'$&III&81.33&$P\bar{4}$&I&112.264&$P_c\bar{4}2c$&IV&81.33&$P\bar{4}$&I\\
\hline
112.265&$P_C\bar{4}2c$&IV&81.33&$P\bar{4}$&I&112.266&$P_I\bar{4}2c$&IV&81.33&$P\bar{4}$&I\\
\hline
113.267&$P\bar{4}2_1m$&I&81.33&$P\bar{4}$&I&113.268&$P\bar{4}2_1m1'$&II&81.33&$P\bar{4}$&I\\
\hline
113.271&$P\bar{4}2_1'm'$&III&81.33&$P\bar{4}$&I&113.272&$P_c\bar{4}2_1m$&IV&81.33&$P\bar{4}$&I\\
\hline
113.273&$P_C\bar{4}2_1m$&IV&81.33&$P\bar{4}$&I&113.274&$P_I\bar{4}2_1m$&IV&81.33&$P\bar{4}$&I\\
\hline
114.275&$P\bar{4}2_1c$&I&81.33&$P\bar{4}$&I&114.276&$P\bar{4}2_1c1'$&II&81.33&$P\bar{4}$&I\\
\hline
114.279&$P\bar{4}2_1'c'$&III&81.33&$P\bar{4}$&I&114.280&$P_c\bar{4}2_1c$&IV&81.33&$P\bar{4}$&I\\
\hline
114.281&$P_C\bar{4}2_1c$&IV&81.33&$P\bar{4}$&I&114.282&$P_I\bar{4}2_1c$&IV&81.33&$P\bar{4}$&I\\
\hline
115.283&$P\bar{4}m2$&I&81.33&$P\bar{4}$&I&115.284&$P\bar{4}m21'$&II&81.33&$P\bar{4}$&I\\
\hline
115.287&$P\bar{4}m'2'$&III&81.33&$P\bar{4}$&I&115.288&$P_c\bar{4}m2$&IV&81.33&$P\bar{4}$&I\\
\hline
115.289&$P_C\bar{4}m2$&IV&81.33&$P\bar{4}$&I&115.290&$P_I\bar{4}m2$&IV&81.33&$P\bar{4}$&I\\
\hline
116.291&$P\bar{4}c2$&I&81.33&$P\bar{4}$&I&116.292&$P\bar{4}c21'$&II&81.33&$P\bar{4}$&I\\
\hline
116.295&$P\bar{4}c'2'$&III&81.33&$P\bar{4}$&I&116.296&$P_c\bar{4}c2$&IV&81.33&$P\bar{4}$&I\\
\hline
116.297&$P_C\bar{4}c2$&IV&81.33&$P\bar{4}$&I&116.298&$P_I\bar{4}c2$&IV&81.33&$P\bar{4}$&I\\
\hline
117.299&$P\bar{4}b2$&I&81.33&$P\bar{4}$&I&117.300&$P\bar{4}b21'$&II&81.33&$P\bar{4}$&I\\
\hline
117.303&$P\bar{4}b'2'$&III&81.33&$P\bar{4}$&I&117.304&$P_c\bar{4}b2$&IV&81.33&$P\bar{4}$&I\\
\hline
117.305&$P_C\bar{4}b2$&IV&81.33&$P\bar{4}$&I&117.306&$P_I\bar{4}b2$&IV&81.33&$P\bar{4}$&I\\
\hline
118.307&$P\bar{4}n2$&I&81.33&$P\bar{4}$&I&118.308&$P\bar{4}n21'$&II&81.33&$P\bar{4}$&I\\
\hline
118.311&$P\bar{4}n'2'$&III&81.33&$P\bar{4}$&I&118.312&$P_c\bar{4}n2$&IV&81.33&$P\bar{4}$&I\\
\hline
118.313&$P_C\bar{4}n2$&IV&81.33&$P\bar{4}$&I&118.314&$P_I\bar{4}n2$&IV&81.33&$P\bar{4}$&I\\
\hline
119.315&$I\bar{4}m2$&I&81.33&$P\bar{4}$&I&119.316&$I\bar{4}m21'$&II&81.33&$P\bar{4}$&I\\
\hline
119.319&$I\bar{4}m'2'$&III&81.33&$P\bar{4}$&I&119.320&$I_c\bar{4}m2$&IV&81.33&$P\bar{4}$&I\\
\hline
120.321&$I\bar{4}c2$&I&81.33&$P\bar{4}$&I&120.322&$I\bar{4}c21'$&II&81.33&$P\bar{4}$&I\\
\hline
120.325&$I\bar{4}c'2'$&III&81.33&$P\bar{4}$&I&120.326&$I_c\bar{4}c2$&IV&81.33&$P\bar{4}$&I\\
\hline
121.327&$I\bar{4}2m$&I&81.33&$P\bar{4}$&I&121.328&$I\bar{4}2m1'$&II&81.33&$P\bar{4}$&I\\
\hline
121.331&$I\bar{4}2'm'$&III&81.33&$P\bar{4}$&I&121.332&$I_c\bar{4}2m$&IV&81.33&$P\bar{4}$&I\\
\hline
122.333&$I\bar{4}2d$&I&81.33&$P\bar{4}$&I&122.334&$I\bar{4}2d1'$&II&81.33&$P\bar{4}$&I\\
\hline
122.337&$I\bar{4}2'd'$&III&81.33&$P\bar{4}$&I&122.338&$I_c\bar{4}2d$&IV&81.33&$P\bar{4}$&I\\
\hline
\textbf{123.339}&$\mathbf{P4/mmm}$&\textbf{I}&\textbf{123.339}&$\mathbf{P4/mmm}$&\textbf{I}&123.340&$P4/mmm1'$&II&83.44&$P4/m1'$&II\\
\hline
123.342&$P4'/mm'm$&III&47.249&$Pmmm$&I&123.343&$P4'/mmm'$&III&47.249&$Pmmm$&I\\
\hline
123.344&$P4'/m'm'm$&III&81.33&$P\bar{4}$&I&123.345&$P4/mm'm'$&III&83.43&$P4/m$&I\\
\hline
123.346&$P4'/m'mm'$&III&81.33&$P\bar{4}$&I&123.348&$P_c4/mmm$&IV&123.339&$P4/mmm$&I\\
\hline
123.349&$P_C4/mmm$&IV&123.339&$P4/mmm$&I&123.350&$P_I4/mmm$&IV&123.339&$P4/mmm$&I\\
\hline
124.351&$P4/mcc$&I&83.43&$P4/m$&I&124.352&$P4/mcc1'$&II&83.44&$P4/m1'$&II\\
\hline
124.354&$P4'/mc'c$&III&83.45&$P4'/m$&III&124.355&$P4'/mcc'$&III&83.45&$P4'/m$&III\\
\hline
124.356&$P4'/m'c'c$&III&81.33&$P\bar{4}$&I&124.357&$P4/mc'c'$&III&83.43&$P4/m$&I\\
\hline
124.358&$P4'/m'cc'$&III&81.33&$P\bar{4}$&I&124.360&$P_c4/mcc$&IV&83.43&$P4/m$&I\\
\hline
124.361&$P_C4/mcc$&IV&83.43&$P4/m$&I&124.362&$P_I4/mcc$&IV&83.43&$P4/m$&I\\
\hline
125.363&$P4/nbm$&I&2.4&$P\bar{1}$&I&125.364&$P4/nbm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
125.366&$P4'/nb'm$&III&2.4&$P\bar{1}$&I&125.367&$P4'/nbm'$&III&2.4&$P\bar{1}$&I\\
\hline
125.368&$P4'/n'b'm$&III&81.33&$P\bar{4}$&I&125.369&$P4/nb'm'$&III&81.33&$P\bar{4}$&I\\
\hline
125.370&$P4'/n'bm'$&III&81.33&$P\bar{4}$&I&125.372&$P_c4/nbm$&IV&2.4&$P\bar{1}$&I\\
\hline
125.373&$P_C4/nbm$&IV&2.4&$P\bar{1}$&I&125.374&$P_I4/nbm$&IV&2.4&$P\bar{1}$&I\\
\hline
126.375&$P4/nnc$&I&2.4&$P\bar{1}$&I&126.376&$P4/nnc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
126.378&$P4'/nn'c$&III&2.4&$P\bar{1}$&I&126.379&$P4'/nnc'$&III&2.4&$P\bar{1}$&I\\
\hline
126.380&$P4'/n'n'c$&III&81.33&$P\bar{4}$&I&126.381&$P4/nn'c'$&III&54.342&$Pc'c'a$&III\\
\hline
126.382&$P4'/n'nc'$&III&81.33&$P\bar{4}$&I&126.384&$P_c4/nnc$&IV&2.4&$P\bar{1}$&I\\
\hline
126.385&$P_C4/nnc$&IV&2.4&$P\bar{1}$&I&126.386&$P_I4/nnc$&IV&2.4&$P\bar{1}$&I\\
\hline
127.387&$P4/mbm$&I&83.43&$P4/m$&I&127.388&$P4/mbm1'$&II&83.44&$P4/m1'$&II\\
\hline
127.390&$P4'/mb'm$&III&47.249&$Pmmm$&I&127.391&$P4'/mbm'$&III&83.45&$P4'/m$&III\\
\hline
127.392&$P4'/m'b'm$&III&81.33&$P\bar{4}$&I&127.393&$P4/mb'm'$&III&83.43&$P4/m$&I\\
\hline
127.394&$P4'/m'bm'$&III&81.33&$P\bar{4}$&I&127.396&$P_c4/mbm$&IV&47.249&$Pmmm$&I\\
\hline
127.397&$P_C4/mbm$&IV&83.43&$P4/m$&I&127.398&$P_I4/mbm$&IV&47.249&$Pmmm$&I\\
\hline
128.399&$P4/mnc$&I&83.43&$P4/m$&I&128.400&$P4/mnc1'$&II&83.44&$P4/m1'$&II\\
\hline
128.402&$P4'/mn'c$&III&83.45&$P4'/m$&III&128.403&$P4'/mnc'$&III&83.45&$P4'/m$&III\\
\hline
128.404&$P4'/m'n'c$&III&81.33&$P\bar{4}$&I&128.405&$P4/mn'c'$&III&83.43&$P4/m$&I\\
\hline
128.406&$P4'/m'nc'$&III&81.33&$P\bar{4}$&I&128.408&$P_c4/mnc$&IV&83.43&$P4/m$&I\\
\hline
128.409&$P_C4/mnc$&IV&83.43&$P4/m$&I&128.410&$P_I4/mnc$&IV&83.43&$P4/m$&I\\
\hline
129.411&$P4/nmm$&I&2.4&$P\bar{1}$&I&129.412&$P4/nmm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
129.414&$P4'/nm'm$&III&2.4&$P\bar{1}$&I&129.415&$P4'/nmm'$&III&2.4&$P\bar{1}$&I\\
\hline
129.416&$P4'/n'm'm$&III&81.33&$P\bar{4}$&I&129.417&$P4/nm'm'$&III&81.33&$P\bar{4}$&I\\
\hline
129.418&$P4'/n'mm'$&III&81.33&$P\bar{4}$&I&129.420&$P_c4/nmm$&IV&2.4&$P\bar{1}$&I\\
\hline
129.421&$P_C4/nmm$&IV&2.4&$P\bar{1}$&I&129.422&$P_I4/nmm$&IV&2.4&$P\bar{1}$&I\\
\hline
130.423&$P4/ncc$&I&2.4&$P\bar{1}$&I&130.424&$P4/ncc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
130.426&$P4'/nc'c$&III&2.4&$P\bar{1}$&I&130.427&$P4'/ncc'$&III&2.4&$P\bar{1}$&I\\
\hline
130.428&$P4'/n'c'c$&III&81.33&$P\bar{4}$&I&\textbf{130.429}&$\mathbf{P4/nc'c'}$&\textbf{III}&\textbf{130.429}&$\mathbf{P4/nc'c'}$&\textbf{III}\\
\hline
130.430&$P4'/n'cc'$&III&81.33&$P\bar{4}$&I&130.432&$P_c4/ncc$&IV&2.4&$P\bar{1}$&I\\
\hline
130.433&$P_C4/ncc$&IV&2.4&$P\bar{1}$&I&130.434&$P_I4/ncc$&IV&2.4&$P\bar{1}$&I\\
\hline
131.435&$P4_2/mmc$&I&47.249&$Pmmm$&I&131.436&$P4_2/mmc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
131.438&$P4_2'/mm'c$&III&2.4&$P\bar{1}$&I&131.439&$P4_2'/mmc'$&III&47.249&$Pmmm$&I\\
\hline
131.440&$P4_2'/m'm'c$&III&81.33&$P\bar{4}$&I&131.441&$P4_2/mm'c'$&III&84.51&$P4_2/m$&I\\
\hline
131.442&$P4_2'/m'mc'$&III&81.33&$P\bar{4}$&I&131.444&$P_c4_2/mmc$&IV&47.249&$Pmmm$&I\\
\hline
131.445&$P_C4_2/mmc$&IV&47.249&$Pmmm$&I&131.446&$P_I4_2/mmc$&IV&47.249&$Pmmm$&I\\
\hline
132.447&$P4_2/mcm$&I&47.249&$Pmmm$&I&132.448&$P4_2/mcm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
132.450&$P4_2'/mc'm$&III&47.249&$Pmmm$&I&132.451&$P4_2'/mcm'$&III&2.4&$P\bar{1}$&I\\
\hline
132.452&$P4_2'/m'c'm$&III&81.33&$P\bar{4}$&I&132.453&$P4_2/mc'm'$&III&84.51&$P4_2/m$&I\\
\hline
132.454&$P4_2'/m'cm'$&III&81.33&$P\bar{4}$&I&132.456&$P_c4_2/mcm$&IV&47.249&$Pmmm$&I\\
\hline
132.457&$P_C4_2/mcm$&IV&47.249&$Pmmm$&I&132.458&$P_I4_2/mcm$&IV&47.249&$Pmmm$&I\\
\hline
133.459&$P4_2/nbc$&I&2.4&$P\bar{1}$&I&133.460&$P4_2/nbc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
133.462&$P4_2'/nb'c$&III&2.4&$P\bar{1}$&I&133.463&$P4_2'/nbc'$&III&2.4&$P\bar{1}$&I\\
\hline
133.464&$P4_2'/n'b'c$&III&81.33&$P\bar{4}$&I&133.465&$P4_2/nb'c'$&III&54.342&$Pc'c'a$&III\\
\hline
133.466&$P4_2'/n'bc'$&III&81.33&$P\bar{4}$&I&133.468&$P_c4_2/nbc$&IV&2.4&$P\bar{1}$&I\\
\hline
133.469&$P_C4_2/nbc$&IV&2.4&$P\bar{1}$&I&133.470&$P_I4_2/nbc$&IV&2.4&$P\bar{1}$&I\\
\hline
134.471&$P4_2/nnm$&I&2.4&$P\bar{1}$&I&134.472&$P4_2/nnm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
134.474&$P4_2'/nn'm$&III&2.4&$P\bar{1}$&I&134.475&$P4_2'/nnm'$&III&2.4&$P\bar{1}$&I\\
\hline
134.476&$P4_2'/n'n'm$&III&81.33&$P\bar{4}$&I&134.477&$P4_2/nn'm'$&III&81.33&$P\bar{4}$&I\\
\hline
134.478&$P4_2'/n'nm'$&III&81.33&$P\bar{4}$&I&134.480&$P_c4_2/nnm$&IV&2.4&$P\bar{1}$&I\\
\hline
134.481&$P_C4_2/nnm$&IV&2.4&$P\bar{1}$&I&134.482&$P_I4_2/nnm$&IV&2.4&$P\bar{1}$&I\\
\hline
135.483&$P4_2/mbc$&I&84.51&$P4_2/m$&I&135.484&$P4_2/mbc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
135.486&$P4_2'/mb'c$&III&2.4&$P\bar{1}$&I&\textbf{135.487}&$\mathbf{P4_2'/mbc'}$&\textbf{III}&\textbf{135.487}&$\mathbf{P4_2'/mbc'}$&\textbf{III}\\
\hline
135.488&$P4_2'/m'b'c$&III&81.33&$P\bar{4}$&I&135.489&$P4_2/mb'c'$&III&84.51&$P4_2/m$&I\\
\hline
135.490&$P4_2'/m'bc'$&III&81.33&$P\bar{4}$&I&135.492&$P_c4_2/mbc$&IV&83.45&$P4'/m$&III\\
\hline
135.493&$P_C4_2/mbc$&IV&84.51&$P4_2/m$&I&135.494&$P_I4_2/mbc$&IV&83.45&$P4'/m$&III\\
\hline
136.495&$P4_2/mnm$&I&47.249&$Pmmm$&I&136.496&$P4_2/mnm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
136.498&$P4_2'/mn'm$&III&47.249&$Pmmm$&I&136.499&$P4_2'/mnm'$&III&2.4&$P\bar{1}$&I\\
\hline
136.500&$P4_2'/m'n'm$&III&81.33&$P\bar{4}$&I&136.501&$P4_2/mn'm'$&III&84.51&$P4_2/m$&I\\
\hline
136.502&$P4_2'/m'nm'$&III&81.33&$P\bar{4}$&I&136.504&$P_c4_2/mnm$&IV&47.249&$Pmmm$&I\\
\hline
136.505&$P_C4_2/mnm$&IV&47.249&$Pmmm$&I&136.506&$P_I4_2/mnm$&IV&47.249&$Pmmm$&I\\
\hline
137.507&$P4_2/nmc$&I&2.4&$P\bar{1}$&I&137.508&$P4_2/nmc1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
137.510&$P4_2'/nm'c$&III&2.4&$P\bar{1}$&I&137.511&$P4_2'/nmc'$&III&2.4&$P\bar{1}$&I\\
\hline
137.512&$P4_2'/n'm'c$&III&81.33&$P\bar{4}$&I&137.513&$P4_2/nm'c'$&III&54.342&$Pc'c'a$&III\\
\hline
137.514&$P4_2'/n'mc'$&III&81.33&$P\bar{4}$&I&137.516&$P_c4_2/nmc$&IV&2.4&$P\bar{1}$&I\\
\hline
137.517&$P_C4_2/nmc$&IV&2.4&$P\bar{1}$&I&137.518&$P_I4_2/nmc$&IV&2.4&$P\bar{1}$&I\\
\hline
138.519&$P4_2/ncm$&I&2.4&$P\bar{1}$&I&138.520&$P4_2/ncm1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
138.522&$P4_2'/nc'm$&III&2.4&$P\bar{1}$&I&138.523&$P4_2'/ncm'$&III&2.4&$P\bar{1}$&I\\
\hline
138.524&$P4_2'/n'c'm$&III&81.33&$P\bar{4}$&I&138.525&$P4_2/nc'm'$&III&56.369&$Pc'c'n$&III\\
\hline
138.526&$P4_2'/n'cm'$&III&81.33&$P\bar{4}$&I&138.528&$P_c4_2/ncm$&IV&2.4&$P\bar{1}$&I\\
\hline
138.529&$P_C4_2/ncm$&IV&2.4&$P\bar{1}$&I&138.530&$P_I4_2/ncm$&IV&2.4&$P\bar{1}$&I\\
\hline
139.531&$I4/mmm$&I&123.339&$P4/mmm$&I&139.532&$I4/mmm1'$&II&87.76&$I4/m1'$&II\\
\hline
139.534&$I4'/mm'm$&III&47.249&$Pmmm$&I&139.535&$I4'/mmm'$&III&47.249&$Pmmm$&I\\
\hline
139.536&$I4'/m'm'm$&III&81.33&$P\bar{4}$&I&139.537&$I4/mm'm'$&III&83.43&$P4/m$&I\\
\hline
139.538&$I4'/m'mm'$&III&81.33&$P\bar{4}$&I&139.540&$I_c4/mmm$&IV&123.339&$P4/mmm$&I\\
\hline
140.541&$I4/mcm$&I&47.249&$Pmmm$&I&140.542&$I4/mcm1'$&II&87.76&$I4/m1'$&II\\
\hline
140.544&$I4'/mc'm$&III&47.249&$Pmmm$&I&140.545&$I4'/mcm'$&III&83.45&$P4'/m$&III\\
\hline
140.546&$I4'/m'c'm$&III&81.33&$P\bar{4}$&I&140.547&$I4/mc'm'$&III&83.43&$P4/m$&I\\
\hline
140.548&$I4'/m'cm'$&III&81.33&$P\bar{4}$&I&140.550&$I_c4/mcm$&IV&47.249&$Pmmm$&I\\
\hline
141.551&$I4_1/amd$&I&2.4&$P\bar{1}$&I&141.552&$I4_1/amd1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
141.554&$I4_1'/am'd$&III&2.4&$P\bar{1}$&I&141.555&$I4_1'/amd'$&III&2.4&$P\bar{1}$&I\\
\hline
141.556&$I4_1'/a'm'd$&III&81.33&$P\bar{4}$&I&141.557&$I4_1/am'd'$&III&88.81&$I4_1/a$&I\\
\hline
141.558&$I4_1'/a'md'$&III&81.33&$P\bar{4}$&I&141.560&$I_c4_1/amd$&IV&2.4&$P\bar{1}$&I\\
\hline
142.561&$I4_1/acd$&I&2.4&$P\bar{1}$&I&142.562&$I4_1/acd1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
142.564&$I4_1'/ac'd$&III&2.4&$P\bar{1}$&I&142.565&$I4_1'/acd'$&III&2.4&$P\bar{1}$&I\\
\hline
142.566&$I4_1'/a'c'd$&III&81.33&$P\bar{4}$&I&142.567&$I4_1/ac'd'$&III&88.81&$I4_1/a$&I\\
\hline
142.568&$I4_1'/a'cd'$&III&81.33&$P\bar{4}$&I&142.570&$I_c4_1/acd$&IV&2.4&$P\bar{1}$&I\\
\hline
\textbf{143.1}&$\mathbf{P3}$&\textbf{I}&\textbf{143.1}&$\mathbf{P3}$&\textbf{I}&\textbf{147.13}&$\mathbf{P\bar{3}}$&\textbf{I}&\textbf{147.13}&$\mathbf{P\bar{3}}$&\textbf{I}\\
\hline
147.14&$P\bar{3}1'$&II&2.5&$P\bar{1}1'$&II&147.16&$P_c\bar{3}$&IV&2.4&$P\bar{1}$&I\\
\hline
148.17&$R\bar{3}$&I&2.4&$P\bar{1}$&I&148.18&$R\bar{3}1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
148.20&$R_I\bar{3}$&IV&2.4&$P\bar{1}$&I&149.23&$P312'$&III&143.1&$P3$&I\\
\hline
150.27&$P32'1$&III&143.1&$P3$&I&156.51&$P3m'1$&III&143.1&$P3$&I\\
\hline
157.55&$P31m'$&III&143.1&$P3$&I&158.59&$P3c'1$&III&143.1&$P3$&I\\
\hline
159.63&$P31c'$&III&143.1&$P3$&I&162.73&$P\bar{3}1m$&I&2.4&$P\bar{1}$&I\\
\hline
162.74&$P\bar{3}1m1'$&II&2.5&$P\bar{1}1'$&II&162.77&$P\bar{3}1m'$&III&147.13&$P\bar{3}$&I\\
\hline
162.78&$P_c\bar{3}1m$&IV&2.4&$P\bar{1}$&I&163.79&$P\bar{3}1c$&I&2.4&$P\bar{1}$&I\\
\hline
163.80&$P\bar{3}1c1'$&II&2.5&$P\bar{1}1'$&II&163.83&$P\bar{3}1c'$&III&147.13&$P\bar{3}$&I\\
\hline
163.84&$P_c\bar{3}1c$&IV&2.4&$P\bar{1}$&I&164.85&$P\bar{3}m1$&I&2.4&$P\bar{1}$&I\\
\hline
164.86&$P\bar{3}m11'$&II&2.5&$P\bar{1}1'$&II&164.89&$P\bar{3}m'1$&III&147.13&$P\bar{3}$&I\\
\hline
164.90&$P_c\bar{3}m1$&IV&2.4&$P\bar{1}$&I&165.91&$P\bar{3}c1$&I&2.4&$P\bar{1}$&I\\
\hline
165.92&$P\bar{3}c11'$&II&2.5&$P\bar{1}1'$&II&165.95&$P\bar{3}c'1$&III&147.13&$P\bar{3}$&I\\
\hline
165.96&$P_c\bar{3}c1$&IV&2.4&$P\bar{1}$&I&166.97&$R\bar{3}m$&I&2.4&$P\bar{1}$&I\\
\hline
166.98&$R\bar{3}m1'$&II&2.5&$P\bar{1}1'$&II&166.101&$R\bar{3}m'$&III&2.4&$P\bar{1}$&I\\
\hline
166.102&$R_I\bar{3}m$&IV&2.4&$P\bar{1}$&I&167.103&$R\bar{3}c$&I&2.4&$P\bar{1}$&I\\
\hline
167.104&$R\bar{3}c1'$&II&2.5&$P\bar{1}1'$&II&167.107&$R\bar{3}c'$&III&2.4&$P\bar{1}$&I\\
\hline
167.108&$R_I\bar{3}c$&IV&2.4&$P\bar{1}$&I&\textbf{168.109}&$\mathbf{P6}$&\textbf{I}&\textbf{168.109}&$\mathbf{P6}$&\textbf{I}\\
\hline
171.121&$P6_2$&I&3.1&$P2$&I&172.125&$P6_4$&I&3.1&$P2$&I\\
\hline
173.129&$P6_3$&I&143.1&$P3$&I&\textbf{174.133}&$\mathbf{P\bar{6}}$&\textbf{I}&\textbf{174.133}&$\mathbf{P\bar{6}}$&\textbf{I}\\
\hline
174.134&$P\bar{6}1'$&II&174.133&$P\bar{6}$&I&174.136&$P_c\bar{6}$&IV&174.133&$P\bar{6}$&I\\
\hline
\textbf{175.137}&$\mathbf{P6/m}$&\textbf{I}&\textbf{175.137}&$\mathbf{P6/m}$&\textbf{I}&\textbf{175.138}&$\mathbf{P6/m1'}$&\textbf{II}&\textbf{175.138}&$\mathbf{P6/m1'}$&\textbf{II}\\
\hline
175.139&$P6'/m$&III&174.133&$P\bar{6}$&I&175.141&$P6'/m'$&III&2.4&$P\bar{1}$&I\\
\hline
175.142&$P_c6/m$&IV&175.137&$P6/m$&I&\textbf{176.143}&$\mathbf{P6_3/m}$&\textbf{I}&\textbf{176.143}&$\mathbf{P6_3/m}$&\textbf{I}\\
\hline
\textbf{176.144}&$\mathbf{P6_3/m1'}$&\textbf{II}&\textbf{176.144}&$\mathbf{P6_3/m1'}$&\textbf{II}&176.145&$P6_3'/m$&III&174.133&$P\bar{6}$&I\\
\hline
176.147&$P6_3'/m'$&III&2.4&$P\bar{1}$&I&176.148&$P_c6_3/m$&IV&176.143&$P6_3/m$&I\\
\hline
177.153&$P62'2'$&III&168.109&$P6$&I&180.171&$P6_22'2'$&III&3.1&$P2$&I\\
\hline
181.177&$P6_42'2'$&III&3.1&$P2$&I&182.183&$P6_32'2'$&III&143.1&$P3$&I\\
\hline
183.189&$P6m'm'$&III&168.109&$P6$&I&\textbf{184.195}&$\mathbf{P6c'c'}$&\textbf{III}&\textbf{184.195}&$\mathbf{P6c'c'}$&\textbf{III}\\
\hline
185.201&$P6_3c'm'$&III&143.1&$P3$&I&186.207&$P6_3m'c'$&III&143.1&$P3$&I\\
\hline
187.209&$P\bar{6}m2$&I&174.133&$P\bar{6}$&I&187.210&$P\bar{6}m21'$&II&174.133&$P\bar{6}$&I\\
\hline
187.213&$P\bar{6}m'2'$&III&174.133&$P\bar{6}$&I&187.214&$P_c\bar{6}m2$&IV&174.133&$P\bar{6}$&I\\
\hline
188.215&$P\bar{6}c2$&I&174.133&$P\bar{6}$&I&188.216&$P\bar{6}c21'$&II&174.133&$P\bar{6}$&I\\
\hline
188.219&$P\bar{6}c'2'$&III&174.133&$P\bar{6}$&I&188.220&$P_c\bar{6}c2$&IV&174.133&$P\bar{6}$&I\\
\hline
189.221&$P\bar{6}2m$&I&174.133&$P\bar{6}$&I&189.222&$P\bar{6}2m1'$&II&174.133&$P\bar{6}$&I\\
\hline
189.225&$P\bar{6}2'm'$&III&174.133&$P\bar{6}$&I&189.226&$P_c\bar{6}2m$&IV&174.133&$P\bar{6}$&I\\
\hline
190.227&$P\bar{6}2c$&I&174.133&$P\bar{6}$&I&190.228&$P\bar{6}2c1'$&II&174.133&$P\bar{6}$&I\\
\hline
190.231&$P\bar{6}2'c'$&III&174.133&$P\bar{6}$&I&190.232&$P_c\bar{6}2c$&IV&174.133&$P\bar{6}$&I\\
\hline
\textbf{191.233}&$\mathbf{P6/mmm}$&\textbf{I}&\textbf{191.233}&$\mathbf{P6/mmm}$&\textbf{I}&191.234&$P6/mmm1'$&II&175.138&$P6/m1'$&II\\
\hline
191.236&$P6'/mm'm$&III&174.133&$P\bar{6}$&I&191.237&$P6'/mmm'$&III&174.133&$P\bar{6}$&I\\
\hline
191.238&$P6'/m'm'm$&III&2.4&$P\bar{1}$&I&191.239&$P6'/m'mm'$&III&2.4&$P\bar{1}$&I\\
\hline
191.240&$P6/mm'm'$&III&175.137&$P6/m$&I&191.242&$P_c6/mmm$&IV&191.233&$P6/mmm$&I\\
\hline
192.243&$P6/mcc$&I&175.137&$P6/m$&I&192.244&$P6/mcc1'$&II&175.138&$P6/m1'$&II\\
\hline
192.246&$P6'/mc'c$&III&174.133&$P\bar{6}$&I&192.247&$P6'/mcc'$&III&174.133&$P\bar{6}$&I\\
\hline
192.248&$P6'/m'c'c$&III&2.4&$P\bar{1}$&I&192.249&$P6'/m'cc'$&III&2.4&$P\bar{1}$&I\\
\hline
192.250&$P6/mc'c'$&III&175.137&$P6/m$&I&192.252&$P_c6/mcc$&IV&175.137&$P6/m$&I\\
\hline
193.253&$P6_3/mcm$&I&176.143&$P6_3/m$&I&193.254&$P6_3/mcm1'$&II&176.144&$P6_3/m1'$&II\\
\hline
193.256&$P6_3'/mc'm$&III&174.133&$P\bar{6}$&I&193.257&$P6_3'/mcm'$&III&174.133&$P\bar{6}$&I\\
\hline
193.258&$P6_3'/m'c'm$&III&2.4&$P\bar{1}$&I&193.259&$P6_3'/m'cm'$&III&2.4&$P\bar{1}$&I\\
\hline
193.260&$P6_3/mc'm'$&III&176.143&$P6_3/m$&I&193.262&$P_c6_3/mcm$&IV&176.143&$P6_3/m$&I\\
\hline
194.263&$P6_3/mmc$&I&176.143&$P6_3/m$&I&194.264&$P6_3/mmc1'$&II&176.144&$P6_3/m1'$&II\\
\hline
194.266&$P6_3'/mm'c$&III&174.133&$P\bar{6}$&I&194.267&$P6_3'/mmc'$&III&174.133&$P\bar{6}$&I\\
\hline
194.268&$P6_3'/m'm'c$&III&2.4&$P\bar{1}$&I&194.269&$P6_3'/m'mc'$&III&2.4&$P\bar{1}$&I\\
\hline
194.270&$P6_3/mm'c'$&III&176.143&$P6_3/m$&I&194.272&$P_c6_3/mmc$&IV&176.143&$P6_3/m$&I\\
\hline
200.14&$Pm\bar{3}$&I&47.249&$Pmmm$&I&200.15&$Pm\bar{3}1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
200.17&$P_Im\bar{3}$&IV&47.249&$Pmmm$&I&201.18&$Pn\bar{3}$&I&2.4&$P\bar{1}$&I\\
\hline
201.19&$Pn\bar{3}1'$&II&2.5&$P\bar{1}1'$&II&201.21&$P_In\bar{3}$&IV&2.4&$P\bar{1}$&I\\
\hline
202.22&$Fm\bar{3}$&I&47.249&$Pmmm$&I&202.23&$Fm\bar{3}1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
202.25&$F_Sm\bar{3}$&IV&47.249&$Pmmm$&I&203.26&$Fd\bar{3}$&I&2.4&$P\bar{1}$&I\\
\hline
203.27&$Fd\bar{3}1'$&II&2.5&$P\bar{1}1'$&II&203.29&$F_Sd\bar{3}$&IV&2.4&$P\bar{1}$&I\\
\hline
204.30&$Im\bar{3}$&I&47.249&$Pmmm$&I&204.31&$Im\bar{3}1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
205.33&$Pa\bar{3}$&I&2.4&$P\bar{1}$&I&205.34&$Pa\bar{3}1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
205.36&$P_Ia\bar{3}$&IV&2.4&$P\bar{1}$&I&206.37&$Ia\bar{3}$&I&2.4&$P\bar{1}$&I\\
\hline
206.38&$Ia\bar{3}1'$&II&2.5&$P\bar{1}1'$&II&215.70&$P\bar{4}3m$&I&81.33&$P\bar{4}$&I\\
\hline
215.71&$P\bar{4}3m1'$&II&81.33&$P\bar{4}$&I&215.73&$P_I\bar{4}3m$&IV&81.33&$P\bar{4}$&I\\
\hline
216.74&$F\bar{4}3m$&I&81.33&$P\bar{4}$&I&216.75&$F\bar{4}3m1'$&II&81.33&$P\bar{4}$&I\\
\hline
216.77&$F_S\bar{4}3m$&IV&81.33&$P\bar{4}$&I&217.78&$I\bar{4}3m$&I&81.33&$P\bar{4}$&I\\
\hline
217.79&$I\bar{4}3m1'$&II&81.33&$P\bar{4}$&I&218.81&$P\bar{4}3n$&I&81.33&$P\bar{4}$&I\\
\hline
218.82&$P\bar{4}3n1'$&II&81.33&$P\bar{4}$&I&218.84&$P_I\bar{4}3n$&IV&81.33&$P\bar{4}$&I\\
\hline
219.85&$F\bar{4}3c$&I&81.33&$P\bar{4}$&I&219.86&$F\bar{4}3c1'$&II&81.33&$P\bar{4}$&I\\
\hline
219.88&$F_S\bar{4}3c$&IV&81.33&$P\bar{4}$&I&220.89&$I\bar{4}3d$&I&81.33&$P\bar{4}$&I\\
\hline
220.90&$I\bar{4}3d1'$&II&81.33&$P\bar{4}$&I&221.92&$Pm\bar{3}m$&I&123.339&$P4/mmm$&I\\
\hline
221.93&$Pm\bar{3}m1'$&II&83.44&$P4/m1'$&II&221.94&$Pm'\bar{3}'m$&III&81.33&$P\bar{4}$&I\\
\hline
221.95&$Pm\bar{3}m'$&III&47.249&$Pmmm$&I&221.97&$P_Im\bar{3}m$&IV&123.339&$P4/mmm$&I\\
\hline
222.98&$Pn\bar{3}n$&I&2.4&$P\bar{1}$&I&222.99&$Pn\bar{3}n1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
222.100&$Pn'\bar{3}'n$&III&81.33&$P\bar{4}$&I&222.101&$Pn\bar{3}n'$&III&2.4&$P\bar{1}$&I\\
\hline
222.103&$P_In\bar{3}n$&IV&2.4&$P\bar{1}$&I&223.104&$Pm\bar{3}n$&I&47.249&$Pmmm$&I\\
\hline
223.105&$Pm\bar{3}n1'$&II&2.5&$P\bar{1}1'$&II&223.106&$Pm'\bar{3}'n$&III&81.33&$P\bar{4}$&I\\
\hline
223.107&$Pm\bar{3}n'$&III&47.249&$Pmmm$&I&223.109&$P_Im\bar{3}n$&IV&47.249&$Pmmm$&I\\
\hline
224.110&$Pn\bar{3}m$&I&2.4&$P\bar{1}$&I&224.111&$Pn\bar{3}m1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
224.112&$Pn'\bar{3}'m$&III&81.33&$P\bar{4}$&I&224.113&$Pn\bar{3}m'$&III&2.4&$P\bar{1}$&I\\
\hline
224.115&$P_In\bar{3}m$&IV&2.4&$P\bar{1}$&I&225.116&$Fm\bar{3}m$&I&123.339&$P4/mmm$&I\\
\hline
225.117&$Fm\bar{3}m1'$&II&83.44&$P4/m1'$&II&225.118&$Fm'\bar{3}'m$&III&81.33&$P\bar{4}$&I\\
\hline
225.119&$Fm\bar{3}m'$&III&47.249&$Pmmm$&I&225.121&$F_Sm\bar{3}m$&IV&123.339&$P4/mmm$&I\\
\hline
226.122&$Fm\bar{3}c$&I&47.249&$Pmmm$&I&226.123&$Fm\bar{3}c1'$&II&87.76&$I4/m1'$&II\\
\hline
226.124&$Fm'\bar{3}'c$&III&81.33&$P\bar{4}$&I&226.125&$Fm\bar{3}c'$&III&47.249&$Pmmm$&I\\
\hline
226.127&$F_Sm\bar{3}c$&IV&47.249&$Pmmm$&I&227.128&$Fd\bar{3}m$&I&2.4&$P\bar{1}$&I\\
\hline
227.129&$Fd\bar{3}m1'$&II&2.5&$P\bar{1}1'$&II&227.130&$Fd'\bar{3}'m$&III&81.33&$P\bar{4}$&I\\
\hline
227.131&$Fd\bar{3}m'$&III&2.4&$P\bar{1}$&I&227.133&$F_Sd\bar{3}m$&IV&2.4&$P\bar{1}$&I\\
\hline
228.134&$Fd\bar{3}c$&I&2.4&$P\bar{1}$&I&228.135&$Fd\bar{3}c1'$&II&2.5&$P\bar{1}1'$&II\\
\hline
228.136&$Fd'\bar{3}'c$&III&81.33&$P\bar{4}$&I&228.137&$Fd\bar{3}c'$&III&2.4&$P\bar{1}$&I\\
\hline
228.139&$F_Sd\bar{3}c$&IV&2.4&$P\bar{1}$&I&229.140&$Im\bar{3}m$&I&123.339&$P4/mmm$&I\\
\hline
229.141&$Im\bar{3}m1'$&II&87.76&$I4/m1'$&II&229.142&$Im'\bar{3}'m$&III&81.33&$P\bar{4}$&I\\
\hline
229.143&$Im\bar{3}m'$&III&47.249&$Pmmm$&I&230.145&$Ia\bar{3}d$&I&2.4&$P\bar{1}$&I\\
\hline
230.146&$Ia\bar{3}d1'$&II&2.5&$P\bar{1}1'$&II&230.147&$Ia'\bar{3}'d$&III&81.33&$P\bar{4}$&I\\
\hline
230.148&$Ia\bar{3}d'$&III&2.4&$P\bar{1}$&I&\textbf{}&$\mathbf{}$&\textbf{}&\textbf{}&$\mathbf{}$&\textbf{}\\
\hline

